RACONTEUR: A Knowledgeable, Insightful, and Portable LLM-Powered Shell Command Explainer

Malicious shell commands are linchpins to many cyber-attacks, but may not be easy to understand by security analysts due to complicated and often disguised code structures. Advances in large language models (LLMs) have unlocked the possibility of generating understandable explanations for shell commands. However, existing general-purpose LLMs suffer from a lack of expert knowledge and a tendency to hallucinate in the task of shell command explanation. In this paper, we present Raconteur, a knowledgeable, expressive and portable shell command explainer powered by LLM. Raconteur is infused with professional knowledge to provide comprehensive explanations on shell commands, including not only what the command does (i.e., behavior) but also why the command does it (i.e., purpose). To shed light on the high-level intent of the command, we also translate the natural-language-based explanation into standard technique & tactic defined by MITRE ATT&CK, the worldwide knowledge base of cybersecurity. To enable Raconteur to explain unseen private commands, we further develop a documentation retriever to obtain relevant information from complementary documentations to assist the explanation process. We have created a large-scale dataset for training and conducted extensive experiments to evaluate the capability of Raconteur in shell command explanation. The experiments verify that Raconteur is able to provide high-quality explanations and in-depth insight of the intent of the command.

==> tables/baseline.tex <==
\begin{table*}[tt]
\centering
\caption{Accuracy of Toxic classification.}
\resizebox{0.8\textwidth}{!}{%

\begin{tabular}{l|lllllc}
\hline
\diagbox[height=2.2em, width=10em]{Method}{Dataset}& Jigsaw & OIG-safety & Beavertails & Jailbreak & HateXplain & MHS  \\ \hline
OpenAI Moderation & 51.70 & 65.85 & 47.95 & 23.3 &  &  \\
Perspective API & 47.72 & 60.56 & 45.95 & 21.74 &  &  \\
Beaver-dam-7b & 89.50 & 47.01 & - & 49.70 &  &  \\
GPT-3.5 & 17.45 & 26.20 & 29.10 & 15.41 & 55.35 &  \\
GPT-4 &  &  &  &  &  &  \\
\sys (Ours) & 88.11 & 94.67 & 84.27 & 88.39 & 82.19 & 90.81 \\ 
\hline
\end{tabular}
}
\label{tab:baseline}
\end{table*}

==> tables/diversified_LLM.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{\small The Performance on Diversified Queries Evaluated by LLMs.}

\footnotesize
\setlength{\tabcolsep}{4mm}{
\begin{tabular}{@{}l|cc|cc|cc@{}}
\toprule
\multirow{2}{*}[-3pt]{Model} & \multicolumn{2}{c|}{Original Query}                                                                                        & \multicolumn{2}{c|}{Diversified Query\tnote{\textdagger}}                                                                                           & \multicolumn{2}{c}{Diversified Query w/ Doc.\tnote{\textdagger}}                                                                                       \\ \cmidrule(l){2-7} 
                       & \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{c|}{GPT-3.5-Turbo}  & \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{c|}{GPT-3.5-Turbo}& \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{c}{GPT-3.5-Turbo} \\ \midrule
GPT-3.5-Turbo          & 9.60$\pm$0.28                        & 9.45$\pm$0.36                       & 8.66$\pm$1.08                        & \textbf{\small9.18$\pm$0.93}         & 7.54$\pm$7.43                        & 9.04$\pm$2.54           \\
GPT-4                  & \textbf{\small9.71$\pm$1.03}         & \textbf{\small9.61$\pm$0.20}        & \textbf{\small9.26$\pm$1.62}         & 9.11$\pm$0.98                        & 8.70$\pm$5.57         & 9.05$\pm$2.31           \\
ChatGLM2-6B            & 6.11$\pm$4.77                        & 7.72$\pm$4.96                       & 5.75$\pm$3.62                        & 6.96$\pm$5.42                        & 5.73$\pm$5.17                        & 7.08$\pm$6.04           \\
\sys                   & 9.34$\pm$0.57                        & 9.57$\pm$0.36                       & 9.03$\pm$1.73                        & 9.10$\pm$2.02                        & \textbf{\small9.03$\pm$2.13}                        & \textbf{\small9.15$\pm$1.24}          \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
% \item[\textdaggerdbl] Malicious Command-Line consists of explanation subsets of \texttt{atomic-red-team}, \texttt{metta}, and \texttt{reverse-shell}.
\item[\textdagger] Diversified Query: the form of the query is converted using Equation~\eqref{equ:aug}.
\end{tablenotes}

\label{tab:diversified_llm}
\end{threeparttable}}
\end{table*}
\raggedbottom


==> tables/evaltask_CCS.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{10pt}%
% \setlength\tabcolsep{4.5pt}
\caption{The Performance on Three Tasks.}

\footnotesize
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
\multirow{2}{*}[-3pt]{Model} & \multicolumn{4}{c|}{Explanation \& Explanation w/ Doc.\tnote{\textdagger}}                                                                                        & \multicolumn{4}{c|}{Multi-Round Interaction}                                                                                           & \multicolumn{4}{c}{Behavior Summarization}                                                                                       \\ \cmidrule(l){2-13} 
                       & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r|}{BLEU-4} & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r|}{BLEU-4} & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r}{BLEU-4} \\ \midrule
GPT-3.5-Turbo          & 49.3                        & 24.0                        & 31.4                        & 28.8                        & \textbf{\small62.3}               & \textbf{\small41.1}               & \textbf{\small51.2}               & \textbf{\small40.5}               & 51.1                        & 26.0                        & 39.5                        & 43.8                       \\
GPT-4                  & 48.5                        & 23.7                        & 32.7                        & 36.9                        & 50.4                        & 26.4                        & 37.3                        & 26.3                        & 44.8                        & 18.2                        & 30.5                        & 42.7                       \\
ChatGLM2-6B            & 46.3                        & 21.9                        & 28.9                        & 31.6                        & 50.2                        & 26.8                        & 36.7                        & 24.7                        & 41.6                        & 15.7                        & 26.8                        & 38.5                       \\
\sys    & \textbf{\small68.4}               & \textbf{\small48.1}               & \textbf{\small54.6}               & \textbf{\small52.9}               & 61.1                        & 40.2                        & 49.0                        & 36.0                        & \textbf{\small70.3}               & \textbf{\small53.9}               & \textbf{\small62.1}               & \textbf{\small63.8}              \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
% \item[\textdaggerdbl] Malicious Command-Line consists of explanation subsets of \texttt{atomic-red-team}, \texttt{metta}, and \texttt{reverse-shell}.
\item[\textdagger] Explanation \& Explanation w/ Doc. include both the explanation task and the explanation with documentation task.
\end{tablenotes}

\label{tab:evaltask}
\end{threeparttable}}
\end{table*}
\raggedbottom


==> tables/evaltask_LLM_CCS.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{10pt}%
% \setlength\tabcolsep{4.5pt}
\caption{The Performance on Three Tasks Evaluated by LLMs.}

\footnotesize
\setlength{\tabcolsep}{4mm}{
\begin{tabular}{@{}l|cc|cc|cc@{}}
\toprule
\multirow{2}{*}[-3pt]{Model} & \multicolumn{2}{c|}{Explanation \& Explanation w/ Doc.\tnote{\textdagger}}                                                                                        & \multicolumn{2}{c|}{Multi-Round Interaction}                                                                                           & \multicolumn{2}{c}{Behavior Summarization}                                                                                       \\ \cmidrule(l){2-7} 
                       & \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{c|}{GPT-3.5-Turbo}  & \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{c|}{GPT-3.5-Turbo}& \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{c}{GPT-3.5-Turbo} \\ \midrule
GPT-3.5-Turbo          & 8.73$\pm$2.20                        & 9.31$\pm$0.50                       & 9.37$\pm$1.40                        & \textbf{\small9.16$\pm$1.36}         & 8.34$\pm$2.14                        & 9.23$\pm$0.60           \\
GPT-4                  & \textbf{\small9.42$\pm$0.87}         & \textbf{\small9.36$\pm$0.73}        & \textbf{\small9.62$\pm$0.48}         & 9.03$\pm$1.83                        & \textbf{\small8.98$\pm$1.35}         & 9.35$\pm$0.55           \\
ChatGLM2-6B            & 5.72$\pm$5.76                        & 7.66$\pm$4.28                       & 7.10$\pm$6.59                        & 7.98$\pm$3.47                        & 7.19$\pm$3.57                        & 8.44$\pm$2.80           \\
\sys                   & 9.17$\pm$1.17                        & 9.31$\pm$0.95                       & 8.40$\pm$3.62                        & 8.69$\pm$2.93                        & 8.86$\pm$1.75                        & \textbf{\small9.41$\pm$0.34}          \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
% \item[\textdaggerdbl] Malicious Command-Line consists of explanation subsets of \texttt{atomic-red-team}, \texttt{metta}, and \texttt{reverse-shell}.
\item[\textdagger] Explanation \& Explanation w/ Doc. include both the explanation task and the explanation with documentation task.
\end{tablenotes}

\label{tab:evaltask_llm}
\end{threeparttable}}
\end{table*}
\raggedbottom


==> tables/existingwork.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{\sys versus existing works.}

% \small
\setlength{\tabcolsep}{3mm}{
\begin{tabular}{@{}rrrcl@{}}
\toprule
\textbf{Method}                              & \textbf{Model Architecture}    & \textbf{Model Parameters} & \textbf{Extra Overhead\tnote{$*$}} & \textbf{Domain}     \\ \midrule
OpenAI Moderation API~\cite{MarkovZANLAJW23} & GPT\tnote{\textdagger}                            & 117M$\sim$1.5B\tnote{\textdagger}                 & $O(n)$                  & General content     \\
Google Perspective API~\cite{PerspectiveAPI} & BERT$\longrightarrow$CNN\tnote{\textdaggerdbl}           & -\tnote{\textdaggerdbl}                         & $O(n)$                  & General content     \\
BeaverDam-7B~\cite{Ji2023BeaverTails}        & LLaMA-7B                          & 7B                        & $O(n)$                  & QA\tnote{\P}                   \\
Wang \textit{et al}.~\cite{WangHACL23}                & GPT-3                          & 175B                      & $O(n)$                  & Hate speech               \\
Cao \textit{et al}.~\cite{Cao2023Toxicity}                & GPT-4, LLaMA2                          & 100T, 13B                      & $O(n)$                  & General content               \\
FakeGPT~\cite{Huang2023Harnessing}           & GPT-3.5                        & $\geq$175B                & $O(n)$                  & Fake news           \\
Ma \textit{et al}.~\cite{Ma2023Adapting}              & ChatGLM2-6B, Baichuan-13B & 6B, 13B                   & $O(n)$                  & General content     \\ \midrule
\textbf{Legilimens (Ours)}                            & \textbf{1$\sim$3-Layer MLP}                            & \textbf{8k$\sim$4.7M}                       & $\mathbf{O(1)}$                  & \textbf{General content, QA\tnote{\P} } \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
\item[] (i) \textdagger: The exact GPT architecture has not been disclosed~\cite{MarkovZANLAJW23}. Based on the publication year~\cite{Yenduri2023Generative} and the API response time, we speculate that it is either GPT-1 or GPT-2. (ii) \textdaggerdbl: The CNNs are distilled from trained BERT-based models. The exact architecture has not been disclosed. (iii) $*$: $n$ denotes the (token) length of input. (iv) \P: ``QA'' refers to moderating question-answering (QA) data to assess the safety of the answers.
% \item[\textdaggerdbl]
% \item[\P] 

\end{tablenotes}

\label{tab:existing}
\end{threeparttable}}
\end{table*}


==> tables/features.tex <==
\begin{table*}[tt]  
\centering 
\caption{Performance Comparison of Different Host LLMs Across Feature Layers}
\begin{threeparttable}
\resizebox{0.9\textwidth}{!}{%  
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}    
\hline    
\multirow{2}{*}{\diagbox[height=2.5em, width=14em]{Feature layers\tnote{1}}{Model}} & \multicolumn{2}{c|}{Chatglm3} & \multicolumn{2}{c|}{Llama2} & \multicolumn{2}{c|}{Falcon} & \multicolumn{2}{c|}{Dolly} & \multicolumn{2}{c}{Vicuna} \\    
\cline{2-11}   
& ACC & AUC & ACC & AUC & ACC & AUC & ACC & AUC & ACC & AUC \\    
\hline    
1 & 85.36 & 0.931 & 87.28 & 0.948 & 86.13 & 0.937 & 81.47 & 0.897 & 85.42 & 0.933 \\    
3 & 85.91 & 0.936 & 87.30 & 0.949 & 85.96 & 0.931 & 81.61 & 0.897 & 85.90 & 0.936 \\    
5 & 85.93 & 0.937 & 87.74 & 0.950 & 86.27 & 0.933 & 79.54 & 0.886 & 86.04 & 0.937 \\    
7 & 86.49 & 0.940 & 87.44 & 0.950 & 86.48 & 0.935 & 77.29 & 0.879 & 85.72 & 0.9342 \\    
9 & 86.57 & 0.941 & 87.76 & 0.950 & 85.93 & 0.932 & 76.33 & 0.869 & 86.39 & 0.9399 \\    
\hline    
\end{tabular}  
}  
\begin{tablenotes}
\raggedright 
\footnotesize  
\item[1] Feature layers represent the hidden layers we select. 
\end{tablenotes}
\end{threeparttable}
\end{table*} 

==> tables/host.tex <==
\begin{table}[tt]    
\centering    
\caption{Comparison of Accuracy of Different Host LLMs in Unseen Jailbreak Dataset Obtained via \sys}
\resizebox{0.45\textwidth}{!}{%    
\begin{tabular}{c|c|c|c|c}      
\hline  
\multicolumn{5}{c}{Unseen Jailbreak Dataset} \\
\hline    
Chatglm3 & Llama2 & Falcon & Dolly & Vicuna \\      
\hline      
83.10 & 84.49 & 80.77 & 77.44 & 81.26 \\      
\hline      
\end{tabular}    
} 

\end{table} 

==> tables/human.tex <==
\begin{table}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{10pt}%
% \setlength\tabcolsep{4.5pt}
\caption{The Overall Performance of the Behavior Explainer on HumanCheck Test Set.}

\footnotesize
\setlength{\tabcolsep}{0.2mm}{
\begin{tabular}{@{}l|cccccc@{}}
\toprule
\multirow{2}{*}[-3pt]{Model} & \multicolumn{6}{c}{HumanCheck}   \\ \cmidrule(l){2-7} 
                       & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r}{BLEU-4} & \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{r}{GPT-3.5-Turbo}                 \\ \midrule
GPT-3.5-Turbo          & 62.1                        & 37.5                        & 45.9                        & 48.8                        & 9.47$\pm$0.53                       & \textbf{\small8.70$\pm$0.87}                 \\
GPT-4                  & 54.4                        & 29.1                        & 36.9                        & 38.8                        & \textbf{\small9.77$\pm$0.37}        & 8.70$\pm$1.08                                \\
ChatGLM2-6B            & 55.7                        & 29.4                        & 34.9                        & 38.3                        & 6.45$\pm$3.23                       & 7.21$\pm$2.64                                \\
\sys                   & \textbf{\small69.6}         & \textbf{\small47.7}         & \textbf{\small53.3}         & \textbf{\small53.6}         & 8.70$\pm$1.86                       & 8.43$\pm$1.28                                \\ \midrule
Increased\tnote{\textdollar} & 25.0\%                      & 62.2\%                      & 52.7\%                      & 39.9\%                      & 34.9\%                              & 16.9\%                                      \\ 
cf. GPT-4\tnote{$\star$} & 127.9\%                     & 163.9\%                     & 144.4\%                     & 138.1\%                     & 89.0\%                              & 96.9\%                                     \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
% \item[\textdaggerdbl] Malicious Command-Line consists of data from \texttt{atomic-red-team}, \texttt{metta}, and \texttt{reverse-shell}.
% \item[\textdagger] Benign Command-Line consists of data from \texttt{NL2Bash}.
\item[\textdollar] Increased: the percentage improvement of \sys over the original ChatGLM2-6B model. 
\item[$\star$] cf. GPT-4: the achieved percentage of GPT-4 performance
\end{tablenotes}

\label{tab:human}
\end{threeparttable}}
\end{table}
\raggedbottom

==> tables/jailbreak.tex <==
\begin{table*}[tt]    
\centering    
\caption{Performance Comparison of Different Host LLMs Across Jailbreak Categories.}
\resizebox{0.95\textwidth}{!}{%    
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}      
\hline      
\multirow{2}{*}{\diagbox[height=2.3em, width=14em]{Jailbreak Categories}{Model}} & \multicolumn{2}{c|}{Chatglm3} & \multicolumn{2}{c|}{Llama2} & \multicolumn{2}{c|}{Falcon} & \multicolumn{2}{c|}{Dolly} & \multicolumn{2}{c}{Vicuna} \\      
\cline{2-11}     
& ACC & AUC & ACC & AUC & ACC & AUC & ACC & AUC & ACC & AUC \\      
\hline      
Pretending & 83.8 & 0.921 & 83.2 & 0.912 & 81.64 & 0.896 & 76.82 & 0.848 & 80.8 & 0.896 \\      
Attention Shifting & 84.38 & 0.924 & 84.53 & 0.923 & 84.3 & 0.920 & 76.50 & 0.847 & 80.33 & 0.891 \\      
Privilege Escalation & 85.5 & 0.933 & 84.93 & 0.928 & 84.17 & 0.918 & 77.7 & 0.860 & 82.68 & 0.910 \\      
Syntactical transformation & 80.83 & 0.890 & 80.87 & 0.893 & 81.73 & 0.900 & 74.14 & 0.824 & 78.2 & 0.868 \\      
\hline      
\end{tabular}    
}    
\end{table*}

==> tables/layer.tex <==
\begin{table*}[tt]  
\centering  
\caption{Performance Comparison of Different Host LLMs Across Classifier Layers}
\resizebox{0.9\textwidth}{!}{  
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}  
\hline  
\multirow{2}{*}{\diagbox[height=2.5em, width=14em]{Classifier layers}{Model}} & \multicolumn{2}{c|}{Chatglm3} & \multicolumn{2}{c|}{Llama2} & \multicolumn{2}{c|}{Falcon} & \multicolumn{2}{c|}{Dolly} & \multicolumn{2}{c}{Vicuna} \\  
\cline{2-11}  
& ACC & AUC & ACC & AUC & ACC & AUC & ACC & AUC & ACC & AUC \\  
\hline  
1 & 79.22 & 0.876 & 85.43 & 0.931 & 83.01 & 0.91 & 76.84 & 0.846 & 82.62 & 0.901 \\  
3 & 85.36 & 0.931 & 87.28 & 0.948 & 86.12 & 0.937 & 81.47 & 0.897 & 85.42 & 0.933 \\  
5 & 84.57 & 0.925 & 87.25 & 0.947 & 85.65 & 0.933 & 81.05 & 0.894 & 85.59 & 0.933 \\  
7 & 77.72 & 0.920 & 84.27 & 0.942 & 84.19 & 0.932 & 77.04 & 0.872 & 82.65 & 0.920 \\  
9 & 82.35 & 0.903 & 86.24 & 0.932 & 84.28 & 0.933 & 51.08 & 0.461 & 81.11 & 0.895 \\  
\hline  
\end{tabular}  
}  
\end{table*}

==> tables/multi-round.tex <==
\begin{table}[tt]\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{\small The Performance of Multi-Round Interaction.}

\footnotesize
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{@{}l|cccc@{}}
\toprule
\multirow{2}{*}[-3pt]{Model}            & \multicolumn{4}{c}{Multi-Round Interaction}                                                                                    \\ \cmidrule(l){2-5} 
                                        & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r}{BLEU-4}      \\ \midrule
GPT-3.5-Turbo                           & \textbf{\small62.3}         & \textbf{\small41.1}         & \textbf{\small51.2}              & \textbf{\small40.5}              \\
GPT-4                                   & 50.4                        & 26.4                        & 37.3                             & 26.3                             \\
ChatGLM2-6B                             & 50.2                        & 26.8                        & 36.7                             & 24.7                             \\
\sys                                    & 61.1                        & 40.2                        & 49.0                             & 36.0                             \\ \midrule
Increased\tnote{\textdollar}            & 21.7\%                      & 50.0\%                     & 33.5\%                           & 45.7\%                         \\ 
cf. GPT-3.5\tnote{$\star$}        & 98.1\%                      & 97.8\%                     & 95.7\%                          & 88.9\%                        \\ \bottomrule
\end{tabular}
}

\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
% \item[\textdaggerdbl] Malicious Command-Line consists of explanation subsets of \texttt{atomic-red-team}, \texttt{metta}, and \texttt{reverse-shell}.
\item[\textdollar] Increased: the percentage improvement of \sys over the original ChatGLM2-6B model. 
\item[$\star$] cf. GPT-3.5: the achieved percentage of GPT-3.5-Turbo performance, since GPT-3.5-Turbo achieves the best performance.
\end{tablenotes}

\label{tab:multiround}
\end{threeparttable}}
\end{table}



==> tables/multilabel.tex <==
\begin{table}[tt]
\begin{threeparttable}
\caption{Performance Comparison of Multi-Label Classification Across Different Feature Layers}

\begin{tabular}{l|llll}

\hline
\multirow{2}{*}{Categories} & \multicolumn{2}{l}{Toxicity\textgreater{}0\tnote{1}} & \multicolumn{2}{l}{Toxicity\textgreater{}0.4\tnote{2}} \\ \cline{2-5} 
                            & layer 1              & layer 3              & layer 1               & layer 3               \\ \hline
Severe Toxicity             & 70.71                & 79.78                &                       &                       \\
Obscene                     & 75.97                & 78.89                &                       &                       \\
Identity Attack             & 77.70                & 79.66                &                       &                       \\
Insult                      & 83.10                & 84.34                &                       &                       \\
Threat                      & 70.27                & 81.93                &                       &                       \\
Sexual Explicit             & 69.54                & 87.92                &                       &                       \\ \hline
\end{tabular}
\begin{tablenotes}
\footnotesize  
\item[1] Toxicity\textgreater{}0 stands for toxic, other is non-toxic.
\item[2] Toxicity\textgreater{}0.4 stands for toxic, other is non-toxic.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/overall_CCS.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{5pt}% 
\setlength{\belowcaptionskip}{10pt}%
% \setlength\tabcolsep{4.5pt}
\caption{The Overall Performance of the Behavior Explainer.}

\footnotesize
\setlength{\tabcolsep}{0.4mm}{
\begin{tabular}{@{}l|cccccc|cccccc@{}}
\toprule
\multirow{2}{*}[-3pt]{Model} & \multicolumn{6}{c|}{Malicious Command-Line\tnote{\textdaggerdbl}}                                                                                        & \multicolumn{6}{c}{Benign Command-Line\tnote{\textdagger}}   \\ \cmidrule(l){2-13} 
                       & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r}{BLEU-4} & \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{r|}{GPT-3.5-Turbo} & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r}{BLEU-4} & \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{r}{GPT-3.5-Turbo} \\ \midrule
GPT-3.5-Turbo          & 48.7                        & 24.3                        & 34.5                        & 36.3                        & 6.74$\pm$7.09                       & 8.66$\pm$2.39                             & 54.3                        & 27.0                        & 35.2                        & 29.5                        & 9.03$\pm$1.06                        & 9.40$\pm$0.59                 \\
GPT-4                  & 45.5                        & 20.3                        & 30.5                        & 40.5                        & 7.94$\pm$6.54                       & \textbf{\small8.79$\pm$1.28}              & 51.8                        & 25.8                        & 36.2                        & 34.2                        & \textbf{\small9.59$\pm$0.69}          & \textbf{\small9.54$\pm$0.28} \\
ChatGLM2-6B            & 42.5                        & 18.0                        & 26.9                        & 35.2                        & 6.11$\pm$4.00                       & 7.59$\pm$4.87                             & 50.5                        & 24.3                        & 32.1                        & 30.9                        & 6.61$\pm$4.72                        & 8.26$\pm$3.59                 \\
\sys                   & \textbf{\small68.9}         & \textbf{\small51.5}         & \textbf{\small58.8}         & \textbf{\small59.5}         & \textbf{\small8.25$\pm$1.82}        & 8.51$\pm$2.41                             & \textbf{\small69.3}       & \textbf{\small69.3}           & \textbf{\small46.1}         & \textbf{\small53.1}         & 8.84$\pm$1.74                        & 9.13$\pm$0.98                 \\ \midrule
Increased\tnote{\textdollar} & 62.1\%                      & 186.1\%                     & 118.5\%                     & 69.0\%                      & 35.0\%                              & 12.1\%                                    & 37.2\%                      & 89.7\%                      & 65.4\%                      & 57.0\%                      & 33.7\%                               & 10.5\%                 \\ 
cf. GPT-4\tnote{$\star$} & 151.4\%                     & 253.7\%                     & 192.8\%                     & 146.9\%                     & 103.9\%                             & 96.8\%                                    & 133.8\%                     & 178.7\%                     & 146.7\%                     & 141.8\%                     & 92.2\%                               & 95.7\%                 \\ \bottomrule

\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
\item[\textdaggerdbl] Malicious Command-Line consists of data from \texttt{atomic-red-team}, \texttt{metta}, and \texttt{reverse-shell}.
\item[\textdagger] Benign Command-Line consists of data from \texttt{NL2Bash}.
\item[\textdollar] Increased: the percentage improvement of \sys over the original ChatGLM2-6B model. 
\item[$\star$] cf. GPT-4: the achieved percentage of GPT-4 performance

\end{tablenotes}

\label{tab:overall}
\end{threeparttable}}
\end{table*}
\raggedbottom

==> tables/overall_NDSS.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{10pt}%
% \setlength\tabcolsep{4.5pt}
\caption{The Overall Performance of the Command Explainer.}

\footnotesize
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
\multirow{2}{*}[-3pt]{Model} & \multicolumn{4}{c|}{Malicious Command\tnote{\textdaggerdbl}}                                                                                        & \multicolumn{4}{c|}{Benign Command\tnote{\textdagger}}                                                                                           & \multicolumn{4}{c}{HumanCheck}                                                                                       \\ \cmidrule(l){2-13} 
                       & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r|}{BLEU-4} & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r|}{BLEU-4} & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r}{BLEU-4} \\ \midrule
GPT-3.5-Turbo          & 48.7                        & 24.3                        & 34.5                        & 36.3                        & 54.3                        & 27.0                        & 35.2                        & 29.5                        & 62.1                        & 37.5                        & 45.9                        & 48.8                       \\
GPT-4                  & 45.5                        & 20.3                        & 30.5                        & 40.5                        & 51.8                        & 25.8                        & 36.2                        & 34.2                        & 54.4                        & 29.1                        & 36.9                        & 38.8                       \\
ChatGLM2-6B            & 42.5                        & 18.0                        & 26.9                        & 35.2                        & 50.5                        & 24.3                        & 32.1                        & 30.9                        & 55.7                        & 29.4                        & 34.9                        & 38.3                       \\
\sys                   & \textbf{\small68.9}                        & \textbf{\small51.5}                        & \textbf{\small58.8}                        & \textbf{\small59.5}                        & \textbf{\small69.3}                        & \textbf{\small46.1}                        & \textbf{\small53.1}                        & \textbf{\small48.5}                        & \textbf{\small69.6}                        & \textbf{\small47.7}                        & \textbf{\small53.3}                        & \textbf{\small53.6}                       \\ \midrule
Increased\tnote{\textdollar} & 62.1\%                      & 186.1\%                     & 118.5\%                     & 69.0\%                      & 37.2\%                              & 89.7\%                                    & 65.4\%                      & 57.0\%                      & 25.0\%                      & 62.2\%                      & 52.7\%                               & 39.9\%                 \\ 
cf. GPT-4\tnote{$\star$} & 151.4\%                     & 253.7\%                     & 192.8\%                     & 146.9\%                     & 133.8\%                     & 178.7\%                     & 146.7\%                     & 141.8\%                     & 127.9\%                               & 163.9\%                 & 144.4\%                               & 138.1\%     \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
\item[\textdaggerdbl] Malicious Command consists of data from \texttt{atomic-red-team}, \texttt{metta}, and \texttt{reverse-shell}.
\item[\textdagger] Benign Command consists of data from \texttt{NL2Bash}.
\item[\textdollar] Increased: the percentage improvement of \sys over the original ChatGLM2-6B model. 
\item[$\star$] cf. GPT-4: the achieved percentage of GPT-4 performance.
\end{tablenotes}

\label{tab:overall}
\end{threeparttable}}
\end{table*}
\raggedbottom

==> tables/overall_NSDI.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{The Overall Performance of the Command Explainer.}

\footnotesize
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
\multirow{2}{*}[-3pt]{Model} & \multicolumn{4}{c|}{Malicious Command-Line\tnote{\textdaggerdbl}}                                                                                        & \multicolumn{4}{c|}{Benign Command-Line\tnote{\textdagger}}                                                                                           & \multicolumn{4}{c}{HumanCheck}                                                                                       \\ \cmidrule(l){2-13} 
                       & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r|}{BLEU-4} & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r|}{BLEU-4} & \multicolumn{1}{r}{ROUGE-1} & \multicolumn{1}{r}{ROUGE-2} & \multicolumn{1}{r}{ROUGE-$\ell$} & \multicolumn{1}{r}{BLEU-4} \\ \midrule
GPT-3.5-Turbo          & 48.7                        & 24.3                        & 34.5                        & 36.3                        & 54.3                        & 27.0                        & 35.2                        & 29.5                        & 62.1                        & 37.5                        & 45.9                        & 48.8                       \\
GPT-4                  & 45.5                        & 20.3                        & 30.5                        & 40.5                        & 51.8                        & 25.8                        & 36.2                        & 34.2                        & 54.4                        & 29.1                        & 36.9                        & 38.8                       \\
ChatGLM2-6B            & 42.5                        & 18.0                        & 26.9                        & 35.2                        & 50.5                        & 24.3                        & 32.1                        & 30.9                        & 55.7                        & 29.4                        & 34.9                        & 38.3                       \\
\sys                   & \textbf{\small68.9}                        & \textbf{\small51.5}                        & \textbf{\small58.8}                        & \textbf{\small59.5}                        & \textbf{\small69.3}                        & \textbf{\small46.1}                        & \textbf{\small53.1}                        & \textbf{\small48.5}                        & \textbf{\small69.6}                        & \textbf{\small47.7}                        & \textbf{\small53.3}                        & \textbf{\small53.6}                       \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
\item[\textdaggerdbl] Malicious Command-Line consists of data from \texttt{atomic-red-team}, \texttt{metta}, and \texttt{reverse-shell}.
\item[\textdagger] Benign Command-Line consists of data from \texttt{NL2Bash}.
\end{tablenotes}

\label{tab:overall}
\end{threeparttable}}
\end{table*}
\raggedbottom

==> tables/physical.tex <==
\begin{table*}\centering
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{Test Sets for Evaluation.}

\small
\setlength{\tabcolsep}{3mm}{
\begin{tabular}{@{}cccccrr@{}}
\toprule
\multicolumn{1}{c}{Type}    & \multicolumn{1}{c}{Data Source} & Language & Task             & Prompt\tnote{\textdagger}      & \#Samples & Alias       \\ \midrule
\multirow{24}{*}{\makecell[c]{Malicious\\Statement}} & \multirow{6}{*}{\texttt{reverse-shell}}  &Chinese      & explanation      & orignal     & 785       & \texttt{rs-zh-ex-or} \\
                            &                                 &Chinese      & explanation      & augment     & 743       & \texttt{rs-zh-ex-au} \\
                            &                                 &Chinese      & explanation      & augment w. doc & 773       & \texttt{rs-zh-ex-ad} \\ \cmidrule(l){3-7} 
                            &                                 &English      & explanation      & orignal     & 954       & \texttt{rs-en-ex-or} \\
                            &                                 &English      & explanation      & augment     & 933       & \texttt{rs-en-ex-au} \\
                            &                                 &English      & explanation      & augment w. doc & 919       & \texttt{rs-en-ex-ad} \\ \cmidrule(l){2-7} 
                            & \multirow{9}{*}{\texttt{metta}}          &Chinese      & explanation      & orignal     & 5         & \texttt{me-zh-ex-or} \\
                            &                                 &Chinese      & explanation      & augment     & 5         & \texttt{me-zh-ex-au} \\
                            &                                 &Chinese      & explanation      & augment w. doc & 8         & \texttt{me-zh-ex-ad} \\ \cmidrule(l){3-7} 
                            &                                 &English      & explanation      & orignal     & 9         & \texttt{me-en-ex-or} \\
                            &                                 &English      & explanation      & augment     & 7         & \texttt{me-en-ex-au} \\
                            &                                 &English      & explanation      & augment w. doc & 10        & \texttt{me-en-ex-ad} \\ \cmidrule(l){3-7} 
                            &                                 &English      & behavior         & orignal     & 196       & \texttt{me-en-be-or} \\
                            &                                 &English      & behavior         & augment     & 212       & \texttt{me-en-be-au} \\
                            &                                 &English      & behavior         & augment w. doc & 323       & \texttt{me-en-be-ad} \\ \cmidrule(l){2-7} 
                            & \multirow{9}{*}{\texttt{atomic-red-team}}       &Chinese      & explanation      & orignal     & 68        & \texttt{rt-zh-ex-or} \\
                            &                                 &Chinese      & explanation      & augment     & 58        & \texttt{rt-zh-ex-au} \\
                            &                                 &Chinese      & explanation      & augment w. doc & 71        & \texttt{rt-zh-ex-ad} \\ \cmidrule(l){3-7} 
                            &                                 &English      & explanation      & orignal     & 66        & \texttt{rt-en-ex-or} \\
                            &                                 &English      & explanation      & augment     & 57        & \texttt{rt-en-ex-au} \\
                            &                                 &English      & explanation      & augment w. doc & 69        & \texttt{rt-en-ex-ad} \\ \cmidrule(l){3-7} 
                            &                                 &English      & behavior         & orignal     & 1464      & \texttt{rt-en-be-or} \\
                            &                                 &English      & behavior         & augment     & 1418      & \texttt{rt-en-be-au} \\
                            &                                 &English      & behavior         & augment w. doc & 1918      & \texttt{rt-en-be-ad} \\ \midrule
\multirow{10}{*}{\makecell[c]{Benign\\Statement}}    & \multirow{10}{*}{\texttt{NL2Bash}}       &Chinese      & explanation      & orignal     & 397       & \texttt{nb-zh-ex-or} \\
                            &                                 &Chinese      & explanation      & augment     & 396       & \texttt{nb-zh-ex-au} \\
                            &                                 &Chinese      & explanation      & augment w. doc & 369       & \texttt{nb-zh-ex-ad} \\ \cmidrule(l){3-7} 
                            &                                 &Chinese      & explanation w. doc & orignal     & 410       & \texttt{nb-zh-ed-or} \\
                            &                                 &Chinese      & explanation w. doc & augment     & 409       & \texttt{nb-zh-ed-au} \\
                            &                                 &Chinese      & explanation w. doc & augment w. doc & 411       & \texttt{nb-zh-ed-ad} \\ \cmidrule(l){3-7} 
                            &                                 &Chinese      & multi-round      & orignal     & 5162      & \texttt{nb-zh-mu-or} \\ \cmidrule(l){3-7} 
                            &                                 &English      & explanation w. doc & orignal     & 386       & \texttt{nb-zh-ed-or} \\
                            &                                 &English      & explanation w. doc & augment     & 396       & \texttt{nb-zh-ed-au} \\
                            &                                 &English      & explanation w. doc & augment w. doc & 407       & \texttt{nb-zh-ed-ad} \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
\item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
\item[\textdagger] original: use the same prompts when querying ChatGPT; augment: use augmented prompts; augment w. doc
\end{tablenotes}

\label{tab:testset}
\end{threeparttable}
\end{table*}

==> tables/prompts.tex <==
\section{Prompts for Different Command Datasets}\label{sec:prompt_dataset}
% ----------- Prompt for Red Team ----------------
\begin{tcolorbox}[title = {Prompt for \texttt{atomic-red-team} \& \texttt{metta} with Meta Information}, colback=white, halign={left}, width=0.9\textwidth, left=2em,parbox=false]
{\small\texttt{Please refer to the English command documentations and command descriptions, explain step by step the meaning of each step and each parameter in the following commands, determine whether the command is potentially malicious code, what type of malicious code it is, and the overall intent of the command, and finally give suggestions on how to dispose of the command.\newline
Command documentation:\newline
\{\}\newline
Command description:\newline
    $~~~~~~$ From MITRE ATT\&CK Technique: \{\}\newline
    $~~~~~~$ cmd name: \{\} \newline
    $~~~~~~$ cmd description: \{\} \newline
Command: `\{\}`}}
\end{tcolorbox}

% % ----------- Prompt for Metta ----------------
% \begin{tcolorbox}[title = {Prompt for \texttt{metta} with Meta Information}, colback=white, halign={left}, width=0.9\textwidth, left=2em,parbox=false]
% {\small\texttt{Please refer to the English command documentations and command descriptions, explain step by step the meaning of each step and each parameter in the following commands, determine whether the command is potentially malicious code, what type of malicious code it is, and the overall intent of the command, and finally give suggestions on how to dispose of the command.\newline
% Command documentation:\newline
% \{\}\newline
% Command description:\newline
%     $~~~~~~$ From MITRE ATT\&CK Technique: \{\}\newline
%     $~~~~~~$ cmd name: \{\} - \{\} \newline
%     $~~~~~~$ cmd description: \{\} \newline
% Command: `\{\}`}
% }
% \end{tcolorbox}


% ----------- Prompt for NL2Bash ----------------
\begin{tcolorbox}[title = {Prompt for \texttt{NL2Bash} with Meta Information}, colback=white, halign={left}, width=0.9\textwidth, left=2em,parbox=false]
{\small\texttt{Please refer to the English command documentations and command descriptions, explain step by step the meaning of each step and each parameter in the following commands, as well as the overall intent of the command.\newline
Command documentation:\newline
\{\}\newline
Command description:\newline
\{\}\newline
Command: `\{\}`}}
\end{tcolorbox}

% ----------- Prompt for Powershell ----------------
\begin{tcolorbox}[title = {Prompt for \texttt{PowerShell} \& \texttt{Unix Shell} with Meta Information}, colback=white, halign={left}, width=0.9\textwidth, left=2em,parbox=false]
{\small\texttt{Explain step by step the meaning of each step and each parameter in the following commands, analyse the overall intent of the command.\newline
Command:`\{\}`\newline}}
\end{tcolorbox}


% ----------- Prompt for ReverseShell ----------------
\begin{tcolorbox}[title = {Prompt for \texttt{reverse-shell} with Meta Information}, colback=white, halign={left}, width=0.9\textwidth, left=2em,parbox=false]
{\small\texttt{Explain step by step the meaning of each step and each parameter in the following commands, determine whether the command is potentially malicious code (specifically, whether it is a reverse shell), analyze the overall intent of the command, and finally give a recommendation on how to dispose of the command.\newline
Command: `\{\}`\newline}}
\end{tcolorbox}
\vfill\eject
\clearpage

% ----------- Prompt for Questions ----------------


==> tables/tasks.tex <==
\begin{table*}\centering
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{Tasks of the Command Explainer.}

\small
\setlength{\tabcolsep}{4mm}{
\begin{tabular}{@{}ccl@{}}
\toprule
Task                                                            & \multicolumn{2}{c}{Examples} \\ \midrule
\multirow{2}{*}[-12pt]{\makecell[c]{Explanation}} 	& {Query}       & \makecell[l]{Explain the following command step by step.\\Command: \codeword{bash -c '0<\&137-;exec ...;sh <\&137 >\&137 2>\&137'}}          \\\cmidrule{2-3}
                                                                & {Response}    & \makecell[l]{Step 1: The command \codeword{bash} is used to ... the flag \codeword{-c} means ...\\Step 2: The parameter \codeword{'0<\&137-;exec ...;sh <\&137 >\&137 2>\&137'} is used to ...\\Overall: The command is potentially malicious ...} \\\midrule
% \multirow{2}{*}[-2pt]{\makecell[c]{Explanation\\(brief)}} 		& {Query}       & \makecell[l]{Give a very brief explanation of the following command.\\Command: \codeword{bash -c '0<\&137-;exec ...;sh <\&137 >\&137 2>\&137'}}       \\\cmidrule{2-3}
                                                                % & {Response}    & \makecell[l]{The given command is ... It opens ... and redirects ...}  \\ \midrule
\multirow{5}{*}[-10pt]{\makecell[c]{Multi-round\\Interaction}} 					& {Query (round 1)}       & \makecell[l]{Command: \codeword{bash -c '0<\&137-;exec ...;sh <\&137 >\&137 2>\&137'}\\What does the command \codeword{bash} do?}       \\\cmidrule{2-3}
                                                                & {Response (round 1)}    & \makecell[l]{The command \codeword{bash} can ...}  \\\cmidrule{2-3}
                                                                & {...}       		& \makecell[l]{\textit{(Multiple rounds of queries and responses ...)}}       \\\cmidrule{2-3}
                                                                & {Query (round k)}       & \makecell[l]{What is the meaning of \codeword{-c}?}       \\\cmidrule{2-3}
                                                                & {Response (round k)}    & \makecell[l]{In \codeword{bash}, \codeword{-c} is used to ...}  \\ \midrule
\multirow{2}{*}[-2pt]{\makecell[c]{Behavior\\Summarization}} 	& {Query}       & \makecell[l]{Very briefly describe what adversaries attempt to do by the following command.\\Command: \codeword{bash -c '0<\&137-;exec ...;sh <\&137 >\&137 2>\&137'}}          \\\cmidrule{2-3}
                                                                & {Response}    & \makecell[l]{Adversaries attempt to ...} \\\bottomrule

\end{tabular}
}


% \begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
% \item[\textdagger] Whether the adversary is informed that indelible watermarking has been adopted.
% \end{tablenotes}

\label{tab:task}
\end{threeparttable}
\end{table*}

==> tables/test_doc_retrieval.tex <==
\begin{table}\centering
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{Documentation Retrieval Performance of Different Text2Vec Models.}

\footnotesize
\setlength{\tabcolsep}{5mm}{
\begin{tabular}{@{}l|c|c|c@{}}
\toprule
\multirow{1}{*}{Model} & \multicolumn{1}{c|}{AUC-ROC} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c}{Precision} 
                       \\ \midrule
Sentence-T5$_{\mathrm{large}}$         & 0.857         & 74.7         & 33.6  \\
GTR-T5$_{\mathrm{XL}}$              & 0.921         & 79.4         & 33.6  \\
SGPT                                & 0.785         & 79.0      & 34.7  \\
E5$_{\mathrm{large}}$               & 0.881         & 77.1         & 34.1  \\
Ours (CD2Vec)                       & \textbf{\small0.981}    & \textbf{\small82.4}    & \textbf{\small35.4}  \\ \bottomrule
\end{tabular}
}


% \begin{tablenotes}[flushleft]
% % \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
% % \item[\textdaggerdbl] Explanation: detailed explanation; Explanation w. Doc: detailed explanation given documentations; Multi-round: multi-round interation; Behavior: behavior summarization.
% % \item[\textdagger] Original Q.: use the same prompts as when requesting ChatGPT; Augmented Q.: use augmented prompts; Augmented Q. w. Doc: use augmented prompts with documentations.
% \end{tablenotes}

\label{tab:test_doc_retrieval}
\end{threeparttable}
\end{table}

==> tables/time.tex <==
\begin{table*}[tt]  
\centering  
\caption{Time consumed for each query.}  
\resizebox{0.9\textwidth}{!}{%  
\begin{tabular}{l|lllllc}  
\hline  
\diagbox[height=2.2em, width=10em]{Dataset}{Method} & OpenAI Moderation & Perspective API & Beaver-dam-7b & GPT-3.5 & GPT-4 & \sys (Ours) \\ \hline  
Jigsaw &  &  &  &  &  &  \\  
OIG-safety &  &  &  &  &  &  \\  
Beavertails &  &  &  &  &  &  \\  
Jailbreak &  &  &  &  &  &  \\  
HateXplain &  &  &  &  &  &  \\  
MHS &  &  &  &  &  &  \\  
Avg.time &  &  &  &  &  &  \\ 
\hline  
\end{tabular}  
}  
\label{tab:time}  
\end{table*} 

==> tables/transfer.tex <==
\begin{table*}\centering
\resizebox{\linewidth}{!}{
\begin{threeparttable}[t]
% \renewcommand{\TPTminimum}{\linewidth}
\setlength{\abovecaptionskip}{0pt}% 
\setlength{\belowcaptionskip}{0pt}%
% \setlength\tabcolsep{4.5pt}
\caption{Tranferability of \sys.}

\scriptsize
% \resizebox{10cm}{!}{
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{@{}ll|cccc|cccc|cccc@{}}
\toprule
\multicolumn{2}{l|}{{Methods}}         		& \multicolumn{4}{c|}{Test on \textbf{BVMR}}        & \multicolumn{4}{c|}{Test on \textbf{SplitNet}}            & \multicolumn{4}{c}{Test on \textbf{SLBR}}                 \\
\multicolumn{2}{l|}{\multirow{2}{*}{Metrics\tnote{\textdagger}}}	& $\mathrm{RMSE}$ & $\mathrm{RMSE}_w$ & $\mathrm{PSNR}$  & $\mathrm{SSIM}$  	& $\mathrm{RMSE}$ & $\mathrm{RMSE}_w$ & $\mathrm{PSNR}$  & $\mathrm{SSIM}$ 				& $\mathrm{RMSE}$ & $\mathrm{RMSE}_w$ & $\mathrm{PSNR}$  & $\mathrm{SSIM}$  \\
\multicolumn{2}{l|}{}							& ($\downarrow$)		& ($\downarrow$)		& ($\uparrow$)	& ($\uparrow$)	& ($\downarrow$)		& ($\downarrow$)		& ($\uparrow$)	& ($\uparrow$)	& ($\downarrow$)		& ($\downarrow$)		& ($\uparrow$)	& ($\uparrow$) \\ \midrule
\multicolumn{1}{l}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Train\\on\end{tabular}}}							& \multicolumn{1}{l|}{\textbf{BVMR}}     				& 0.9558      & 3.5584      & 50.61     & 0.9993    & 0.6594      & 3.6217      & 53.37     & 0.9997    & 0.8483      & 6.7713      & 53.07     & 0.9988    \\
												& \multicolumn{1}{l|}{\textbf{SplitNet}~} & 2.2618      & 33.3447     & 42.06     & 0.9888    & 0.5013      & 0.9306      & 55.64     & 0.9998    & 1.9896      & 35.4236     & 44.33     & 0.9876    \\
												& \multicolumn{1}{l|}{\textbf{SLBR}}     & 1.0957      & 5.2673      & 49.26     & 0.9990     & 0.6604      & 3.5847      & 53.24     & 0.9997    & 0.6284      & 3.7813      & 55.79     & 0.9994    \\ \bottomrule
\end{tabular}
}


\begin{tablenotes}[flushleft]
% \item[] \vspace{-1pt}\hspace{-2pt}\footnotesize $^\dagger$
\item[\textdagger] $\mathrm{RMSE}$, $\mathrm{RMSE}_w$, $\mathrm{PSNR}$, and $\mathrm{SSIM}$ compare the recovered images with the watermarked images.
\end{tablenotes}

\label{tab:transfer}
\end{threeparttable}}
\end{table*}

==> tables/unseen_dataset.tex <==
\begin{table}[tt]
\begin{threeparttable} 
\caption{11}

\begin{tabular}{l|lll}

\hline
\multirow{2}{*}{Original Dataset} & \multicolumn{3}{c}{Unseen Dataset} \\ \cline{2-4} 
& OIG-Safety  & HateXplain  & MHS  \\ \hline
Jigsaw and HateXplain                      & 70.27                & 81.93                &                          \\
Jigsaw and MHS    & 69.54     & 87.92 &   \\ \hline
\end{tabular}\label{tab:unseen}
\begin{tablenotes}
\footnotesize  
\item[1] 
\item[2] 
\end{tablenotes}
\end{threeparttable}
\end{table}

